Fair Incentivization of Bandwidth Sharing in Decentralized Storage Networks

Peer-to-peer (p2p) networks are not independent of their peers, and the network efficiency depends on peers contributing resources. Because shared resources are not free, this contribution must be rewarded. Peers across the network may share computation power, storage capacity, and bandwidth. This paper looks at how bandwidth incentive encourages peers to share bandwidth and rewards them for their contribution. With the advent of blockchain technology, many p2p networks attempt to reward contributions by crypto-assets. We conduct simulations to better understand current incentive mechanisms, assess the fairness of these mechanisms, and to look for ways to make those incentives more equitable. The following are the primary contributions of this study: (i) We investigate and simulate bandwidth incentives within Swarm, a cutting-edge p2p storage network; (ii) We demonstrate one approach to make the current bandwidth incentives more equitable; (iii) We use the Gini coefficient to define two quantifiable fairness characteristics to evaluate reward sharing in a decentralized p2p storage network.

==> tex/background.tex <==
\section{Background and Motivation}
In this section, we present the system model (\ref{subsec:sysmodel}) \veg{system model does not belong to this section}, define problems in P2P networks (\ref{subsec:problems}), overview the bandwidth incentives (\ref{subsec:bandwidthoverview}), 
and define forwarding Kademlia (\ref{subsec:forwarding_kademlia}).

% system model should not be here. check NSDI to see where it goes.
%\input{tex/system_model.tex}
\input{tex/bandwidth_incentives_overview.tex}
\input{tex/forwarding_kademlia.tex}
\input{tex/swarm.tex}

==> tex/bandwidth_incentives.tex <==
\section{Bandwidth Incentives}
\label{sec:bandwidth}
In this section, we give an overview of the bandwidth incentives in Swarm one of the most cutting-edge p2p storage networks.
Swarm is a decentralized p2p storage network with its own token named bzz.
With built-in incentives for bandwidth and storage sharing, Swarm will be self-sustaining \cite{bookofswarm}. 

The bandwidth incentives in the Swarm network are built by combining three components. One of them is in charge of calculating a peer's 
relative bandwidth contribution. If one node has utilized much more bandwidth than the others, 
the other two work together to pay the debt.

\textbf{Swarm Accounting Protocol}

Peers in the Swarm network keep an accounting balance with the connected nodes from their routing table. Every peer keeps track of the 
bandwidth it provides and receives in relation to other peers.
Consider the case when peer \textit{d} wishes to download a file and sends a chunk request to another peer \textit{f} with which it is 
connected. Peer \textit{d} is aware of its debt to node \textit{f} after delivering the chunk.
Peer \textit{f} on the opposite side of the connection keeps track of the bandwidth used. This mechanism is called SWAP (Swarm Accounting 
Protocol)\cite{tronswap}. Many sent pieces make up a routine operation in the Swarm network. Peers update their p2p accounting balance with 
others once the service is given. This change could result in a zero swap balance, meaning bandwidth providers will cancel each other's debt. 
In the Swarm network, the SWAP mechanism allows for service-to-service exchange.

\textbf{Large debt settlement}

What happens if a peer's SWAP balance has a big debt? The network enabled bzz to settle its high positive balances.
SWAP is designed to eliminate debts between forwarder nodes, or nodes that assist in downloading or uploading by transferring requests and data 
chunks.
A request's originator is expected to have a substantial negative balance with other nodes, making reciprocal action impossible to cancel. It 
is necessary to pay off the debt before using the network's services again. 
As a result, they can pay other nodes or wait a specific length of time to bring the balance to zero.

\textbf{Time-based forgiveness}

Peers forgive each other's debts over time in the Swarm network. This means that each network peer provides a certain amount of bandwidth for 
free.
This feature enables peers to connect to the network and request content for free, but at a slow speed.

\textbf{Chequebook contract}

The p2p settlement happens all the time inside the Swarm network, but for security reasons, money is never exchanged between the forwarder nodes. 
Request originators that wish to use the service right away and not wait for time-based amortization will shortly reach the debt settlement threshold and will need to pay the debt. 
Payments can be made with bzz, but posting all transactions to the blockchain slows down and limits scalability. As a result, Swarm offers a cheque-based settlement. 
Only originators can issue a cheque in this manner, and only forwarders in the zero proximity order will receive a cheque payment in return for their bandwidth contribution.
%Cheque settlements?




==> tex/bandwidth_incentives_overview.tex <==
\subsection{Bandwidth incentives overview}
\label{subsec:bandwidthoverview}
Bandwidth is one of the resources used for P2P networks and is vital for message-passing and file sharing. It is essential to find a way to compensate nodes for their bandwidth sharing and encourage them to continue. 
For example, it is critical to have relay nodes in the Tor network. Several works have been done to present mechanisms for compensating volunteer relay 
nodes\cite{10.1007/978-3-540-70630-4_14,10.1145/1655188.1655195,10.1007/978-3-642-14577-3_19,10.1145/2076732.2076762,Johnson2013OnionsFS}, but none of them yet widely adopted.

==> tex/forwarding_kademlia.tex <==
\subsection{Forwarding Kademlia}
\label{subsec:forwarding_kademlia}
Kademlia\cite{10.1007/3-540-45748-8_5} is a structured overlay network deployed by several P2P networks (i.e., BitTorrent and eMule). The protocol provides efficient key-based routing by using the XOR metric to find the distance between points 
in the identifier space. Each node in the network chooses a unique nodeId from the id space and maintains a routing table with nodeIds of neighbors from the overlay topology. In this way, the identifier space is 
divided between nodes, and every node is responsible for a particular range. This way, successively forwarding a message to neighbors with closer nodeId to a destination key works efficiently. In original Kademlia nodes, 
choose a random 160-bit nodeId and build the routing table with 160 k-buckets. Every bucket can have at most k entries, including (IP address, UDP port, NodeId) of others. A binary tree is generated with buckets, 
and nodes get assigned to buckets based on the shortest unique prefix of their nodeIds. When a node wants to find a target key, the node generates an RPC to the nodes inside the closest bucket to the destination. 
Then, the subsequent RPCs are to nodes returned by the previous RPC. Each step goes closer to the destination in a logarithmic way. There is a problem in this approach that reveals the identity of the original requestor. 
Forwarding Kademlia, which Swarm uses, removes this problem by not returning the RPC results to the first node. In forwarding Kadmlia, a node receives a request from another node and forwards it to the closer nodes while 
it does not know if the previous node is the originator of the request or just a forwarder like herself.

==> tex/problems.tex <==
\section{Problem description}
\label{sec:problems}
In this section, we go over the major roadblocks that prevented p2p networks from becoming widely used. 

\textbf{Problem 1: Lack of incentives and free riding}. It is difficult to locate peers who are willing to donate their resources, such as storage and bandwidth, for free. Peers typically aim to reduce their contribution while getting the most out of the network. Free riding is a 
problem that has been widely documented in old p2p networks such as Gnutella\cite{Adar_Huberman_2000}. BitTorrent attempted to solve the problem of free riders by introducing an incentive layer (tit-for-tat). With the incentive layer, peers only contribute when they are given anything in return. However, this restriction only applies during the download procedure. 

\textbf{Problem 2: Instability, heterogenity and churn}.
Problem 1 results in high levels of heterogeneity and churn. Nodes joining and leaving these networks on a regular basis can cause performance and latency issues, when opposed to p2p networks, stable cloud servers provide higher service quality. 


%Problem 1: Lack of incentives and free riding}. It is not easy to find users who share their resources, 
%including storage and bandwidth, for free. Typically, users try to minimize their contribution while obtaining the maximum from the network. A problem called free riding and extensively 
%reported in old P2P networks such as Gnutella\cite{Adar_Huberman_2000}. BitTorrent tried to eliminate the free riding problem by adding an incentive layer (tit-for-tat). 
%Peers only reciprocate contribution. But, this enforcement only works during the download process.

%\textbf{Problem 2: Instability, heterogenity and churn}.
%Problem 1 concludes in high heterogeneity and high churn. Constant join and leave of nodes to these networks can cause performance problems and latency. 
%Stable cloud servers show better quality of service compared to P2P networks.


==> tex/system_model.tex <==
\section{System model}
\label{sec:sysmodel}
We assume a decentralized p2p system model of a network composed of a set of $n$ peers, where peers are connected to each other in a p2p way. Each 
node is connected to a small set of nodes with directed links.
Peers can both initiate a download request and forward a request by message-passing. Peers communicate by exchanging messages and are correct, 
which means they do not fail and do not experience arbitrary 
behavior (i.e., no Byzantine failures). 
A peer can originate a download request. For downloading a file, peer \textit{p} generates the required amount of requests to collect all data 
chunks. Data chunks are distributed in the network. Peer \textit{s} stores a data 
chunk and all nodes in between, helping with forwarding the download request and delivering back the requested data chunk. Communication 
happens by exchanging messages over a set of directed links using 
primitives \textit{download(c, d)} and \textit{deliver(f, d)}, where \textit{c} is the address of the closest node to data chunk \textit{d}, 
and \textit{f} is the forwarder's address. We assume communication links are reliable, 
which guarantees delivery of a request if both sender and receiver are correct. In addition to that, a request is received at most once, and 
only if it was previously sent.
